Toward Organizational Decoupling in Microservices Through Key Developer Allocation

With microservices continuously being popular in the software architecture domain, more practitioners and researchers have begun to pay attention to the degradation issue that diminishes its sustainability. One of the key factors that causes the degradation of the architecture is that of the software architectural structure according to Conway's law. However, the best practice of "One microservice per Team", advocated widely by the industry, is not commonly adopted, especially when many developers contribute heavily across multiple microservices and create organizational coupling. Therein, many key developers, who are responsible for the majority of the project work and irreplaceable to the team, can also create the most coupling and be the primary cause of microservice degradation. Hence, to properly maintain microservice architecture in terms of its organizational structure, we shall identify these key developers and understand their connections to the organizational coupling within the project. We propose an approach to identify the key developers in microservice projects and investigate their connection to organizational coupling. The approach shall facilitate the maintenance and optimization of microservice projects against degradation by detecting and mitigating organizational coupling.

==> archive.tex <==
%%%%%% Table II (removed for space) %%%%%%
\begin{table*}[!ht]
    \centering
    \adjustbox{max width=\textwidth}{
    \begin{tabular}{l|l|l|l}
    \hline 
       \textbf{Service} & \textbf{Jack} & \textbf{Maven} & \textbf{Connector} \\
    \hline 
audit	&	[('arpXXX', 0.62), ('ragXXX', 0.6), ('gauXXX', 0.51)]	&	[('arpXXX', 1.0)]	&	[('arpXXX', 0.62), ('ragXXX', 0.6), ('gauXXX', 0.51)]	\\
authentication	&	[('sunXXX', 0.33), ('shuXXX', 0.27), ('yesXXX', 0.22)]	&	[('ragXXX', 0.4), ('shuXXX', 0.4), ('sunXXX', 0.2)]	&	[('sunXXX', 0.33), ('shuXXX', 0.27), ('yesXXX', 0.22)]	\\
bpmn	&	[('shuXXX', 0.12), ('yesXXX', 0.06), ('ragXXX', 0.06)]	&	[('shuXXX', 0.71), ('yesXXX', 0.29)]	&	[('shuXXX', 0.12), ('yesXXX', 0.06), ('ragXXX', 0.06)]	\\
chat	&	[('surXXX', 0.18), ('shuXXX', 0.16), ('ragXXX', 0.05)]	&	[('surXXX', 1.0)]	&	[('surXXX', 0.18), ('shuXXX', 0.16), ('ragXXX', 0.05)]	\\
feature	&	[('shuXXX', 0.1), ('yesXXX', 0.09), ('ragXXX', 0.06)]	&	[('yesXXX', 0.5), ('shuXXX', 0.5)]	&	[('shuXXX', 0.1), ('yesXXX', 0.09), ('ragXXX', 0.06)]	\\
in-mail	&	[('shuXXX', 0.19), ('yesXXX', 0.05), ('ragXXX', 0.05)]	&	[('shuXXX', 0.92), ('yesXXX', 0.08)]	&	[('shuXXX', 0.19), ('yesXXX', 0.05), ('ragXXX', 0.05)]	\\
notification	&	[('shuXXX', 0.13), ('yesXXX', 0.06), ('ragXXX', 0.06)]	&	[('shuXXX', 0.71), ('yesXXX', 0.29)]	&	[('shuXXX', 0.13), ('yesXXX', 0.06), ('ragXXX', 0.06)]	\\
payment	&	[('shiXXX', 0.29), ('ragXXX', 0.23), ('arpXXX', 0.23)]	&	[('shiXXX', 0.6), ('shuXXX', 0.4)]	&	[('shiXXX', 0.29), ('ragXXX', 0.23), ('arpXXX', 0.23)]	\\
reporting	&	[('shuXXX', 0.12), ('yesXXX', 0.06), ('surXXX', 0.06)]	&	[('shuXXX', 1.0)]	&	[('shuXXX', 0.12), ('yesXXX', 0.06), ('surXXX', 0.06)]	\\
scheduler	&	[('sunXXX', 0.22), ('ragXXX', 0.22), ('arpXXX', 0.22)]	&	[('yesXXX', 0.67), ('shuXXX', 0.33)]	&	[('sunXXX', 0.22), ('ragXXX', 0.22), ('arpXXX', 0.22)]	\\
search	&	[('shuXXX', 0.14), ('ragXXX', 0.07), ('arpXXX', 0.07)]	&	[('shuXXX', 0.83), ('surXXX', 0.17)]	&	[('shuXXX', 0.14), ('ragXXX', 0.07), ('arpXXX', 0.07)]	\\
user	&	[('sunXXX', 0.24), ('ragXXX', 0.22), ('arpXXX', 0.22)]	&	[('shuXXX', 0.88), ('sunXXX', 0.12)]	&	[('sunXXX', 0.24), ('ragXXX', 0.22), ('arpXXX', 0.22)]	\\
video	&	[('shiXXX', 0.21), ('sunXXX', 0.2), ('ragXXX', 0.2)]	&	[('yesXXX', 0.33), ('shuXXX', 0.33), ('shiXXX', 0.33)]	&	[('shiXXX', 0.21), ('sunXXX', 0.2), ('ragXXX', 0.2)]	\\
    \hline
Whole	&	[('shuXXX', 0.12), ('sunXXX', 0.08), ('aksXXX', 0.07), 	&	[('shuXXX', 0.4), ('sunXXX', 0.2), ('arpXXX', 0.16),	&	[('shuXXX', 0.12), ('sunXXX', 0.08), ('aksXXX', 0.07), 	\\
Project	&	('arpXXX', 0.07), ('yesXXX', 0.07), ('395XXX', 0.06),	&	 ('shiXXX', 0.09), ('surXXX', 0.06), ('ragXXX', 0.03), 	&	('arpXXX', 0.07), ('yesXXX', 0.07), ('395XXX', 0.06),	\\
	&	 ('shiXXX', 0.06), ('barXXX', 0.06), ('ragXXX', 0.06), 	&	('496XXX', 0.02), ('yesXXX', 0.01), ('devXXX', 0.01), 	&	('shiXXX', 0.06), ('barXXX', 0.06), ('ragXXX', 0.06), 	\\
	&	('surXXX', 0.05)]	&	('mayXXX', 0.01)]	&	('surXXX', 0.05)]	\\
    \hline
    \end{tabular}
    }
    \caption{The Key Developers of Each Microservice and Whole Project (2023-11-21)}
    \label{tab:kd2023}
\end{table*}
